Multi-Modal MPPI and Active Inference for Reactive Task and Motion Planning

Task and Motion Planning (TAMP) has made strides in complex manipulation tasks, yet the execution robustness of the planned solutions remains overlooked. In this work, we propose a method for reactive TAMP to cope with runtime uncertainties and disturbances. We combine an Active Inference planner (AIP) for adaptive high-level action selection and a novel Multi-Modal Model Predictive Path Integral controller (M3P2I) for low-level control. This results in a scheme that simultaneously adapts both high-level actions and low-level motions. The AIP generates alternative symbolic plans, each linked to a cost function for M3P2I. The latter employs a physics simulator for diverse trajectory rollouts, deriving optimal control by weighing the different samples according to their cost. This idea enables blending different robot skills for fluid and reactive plan execution, accommodating plan adjustments at both the high and low levels to cope, for instance, with dynamic obstacles or disturbances that invalidate the current plan. We have tested our approach in simulations and real-world scenarios.

==> tex/old/discussion.tex <==
\section{Discussion and Future work}
\label{sec:discussion}
\mycyan{Add here possible weaknesses and future work, or reasons behind specific choices}

\begin{itemize}
    \item How are the different parts of the cost normalized/weighted? 
    %\item What is the difference between the active inference free energy and the MPPI free energy? Why not use one only? It is easier to solve the low level by sampling over a cost function instead of defining a differentiable cost. Some constraints, such as collision constraints, are difficult to define in a differentiable form.
    \item Can we use the confidence over a prior input to decide the number of samples at runtime? Ideally, if the control prior is 100\% sure we could just have one sample, the mean itself.
    \item Learn specific policies or priors associated with a certain cost function and then keep them in a sort of memory? Online learning without forgetting successfully sampled trajectories? 
\end{itemize}

% \textbf{Differences between our approach and classical TAMP}
% In our approach, both the high-level decision and the low-level motions are continuously performed during operations, while classical TAMP first finds a solution in terms of plan skeleton and associated action constraints, and then executes it. 

% Additionally, TAMP is concerned with finding a plan skeleton to complete the task and its parameters. In our work, a partial skeleton containing desired states (and not actions) is provided, roughly encoding the task to be performed. At runtime, the skeleton is adapted by active inference, which selects the necessary costs to be minimized in order to reach the desired state departing from the current one. Then, instead of sampling high-level action parameters as commonly done in TAMP, the MPPI samples low-level control actions (i.e. torques) on the basis of the prior controllers that can minimize the current cost. 

% In TAMP, the constraints are added to the action templates. In our case, the constraints for action depend on the current cost. This increases the flexibility in executing single actions in different ways and unlocks the possibility of using learned policies. By fusing controllers, one can use a learned policy in combination with additional constraints such as collision avoidance by including it in the cost to be minimized, something not possible in classical TAMP, where in the best case the learned policy can just be executed as it is or not used at all if all motions are based on a single motion planner. 

==> tex/old/previous_work.tex <==

The authors in \cite{rana2020multiplicative} presented a Multiplicative Controllers Fusion approach (MCF). This method can fuse a classical controller, such as artificial potential fields, with a stochastic RL policy for guided exploration and deployment. During training, MCF employs a gating function as a reverse logistic function of the training steps taken. This allows to rely more on the prior controller at the beginning of the training, and then let the policy approach the optimal solution. During deployment, the uncertainty in the policy and in the classical controller are used to weight their contribution in the control input. Doing so, the policy can transfer to the real world by falling back to the prior controller in uncertain states. The experiments in \cite{rana2020multiplicative} shows that fusing classical controllers and learned policies improves the learning step and allows to safely deploy the learned policy from simulation to real world without fine tuning. In a follow up  work\cite{rana2021bayesian}, the same authors improved their method by using epistemic uncertainty estimation techniques to replace the gating function in \cite{rana2020multiplicative}. Tuning the gating function can be tedious and it requires to find the correct balance. Despite the great experimental results in \cite{rana2021bayesian} which showcase how controllers fusion can combine the complementary strengths of deep RL and classical controllers, we find several limitations in \cite{rana2020multiplicative, rana2021bayesian}, some of which we consider fundamental. 

In particular, both methods require a measure of uncertainty of the controllers. This required the training of an ensemble of $M$ policies for the same task as well as a Monte Carlo sampling to estimate the uncertainty for a deterministic controller. Another problem of fusing controllers based on their respective uncertainties, as pointed out by the authors themselves \cite{rana2021bayesian}, is that when both the classical controller and policy are confident on different actions (both valid for a task), the result is a stagnation of the control input. Besides this, the main limitation we see is that fusion of controllers in this manner can only happen between two controllers that want to achieve the same objective. It is not possible with the methods in \cite{rana2020multiplicative,rana2021bayesian} to fuse controllers for different goals because by definition the fusion is done considering the uncertainty of the controllers for the same goal. In other words, it would be impossible to fuse a reactive controller for collision avoidance with a policy for opening a door which was not trained to avoid obstacles. 

In our work we overcome these limitations, allowing to fuse controllers for different task, removing the need to compute controller's and policy's uncertainties, and removing the risk of stagnation of the control input. 



==> tex/old/related_work.tex <==
\section{Related work}
In this section, we report relevant works with a focus on reactive TAMP and Sampling-based MPC. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Previous Work: a thorough literature study has been performed (complete scan of
% the most important conferences/journals in the relevant domain of the past 2
% years, relevant references of references, etc.)

% Previous Work: meaningful structuring of discussion according to the criteria of
% main contributions. No intermingling previous vs. proposed approach. Description
% of previous work is such that difference with current work is evident and relevant
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Reactive TAMP}
In \cite{toussaint2022sequence}, the authors provide a reactive MPC strategy to execute a TAMP plan as a given linear sequence of constraints. Instead of composing primitive skills, \cite{toussaint2022sequence} derive the control law from a composition of constraints for MPC. The reactive nature of the approach allows coping with disturbances and dynamic collision avoidance during the execution of a TAMP plan. The work in \cite{migimatsu2020object} formulates a TAMP plan in object-centric Cartesian coordinates, showing how this allows coping with perturbations such as moving a target location. Both \cite{toussaint2022sequence, migimatsu2020object}, however, do not consider adaptation at the symbolic action level if a perturbation invalidates the current plan. 

On the other hand, a number of papers focused on adapting and repairing high-level action sequences during execution. Authors in \cite{Paxton2019} propose to represent robot task plans as robust logical-dynamical systems. The method can effectively adapt the logic plan in order to deal with external human disturbances. Similarly, \cite{harris2022fc} presented a method to coordinate control chains and achieved robust plan execution through plan switching and controller selection. \cite{Colledanchise2019} proposed instead to blend task and action planners by dynamically expanding a behavior tree at runtime through back-chaining. Similarly, \cite{zhou22} presents a reactive task allocation framework based on behavior trees and linear temporal logic for multi-robot systems. In \cite{li2021reactive}, behavior trees and linear temporal logic have been combined into a reactive TAMP method against a cooperative or adversarial human operator which might invalidate the current plan. A recent work \cite{huang2022parallel} proposes to use Monte Carlo Tree Search in combination with Isaac Gym to speed up task planning for multi-step object retrieval from clutter, where complex physical interaction is required. This is a promising direction, but \cite{huang2022parallel} only focuses on high level reasoning and executes pre-defined motions in open-loop. 

In our previous work \cite{pezzato2022aipbt}, active inference and behavior tree were combined to provide reactive action selection in long-term tasks in partially observable and dynamic environments. This method achieves hierarchical deliberation and continual online planning, which makes it particularly appealing for the problem of reactive TAMP at hand. In this paper, we extend \cite{pezzato2022aipbt} bridging the gap to low-level reactive control by planning cost functions instead of symbolic actions.  

% All these works propose effective solutions but the focus is mainly on the adaptation of the high-level plan. 


% In fact, recent works \cite{lee2022hierarchical, jaquier22} focused specifically on sequencing and blending skills for a more fluid execution. 

\paragraph{Sampling-based MPC}

In order for the robot to robustly operate in dynamic and uncertain environments, it must react to new situations with intelligent decision-making and fast execution. Model Predictive Control (MPC) addresses this problem via constrained optimization in a receding horizon way and has been widely used on real robotic systems \cite{bangura2014real, erez2013integrated, scianca2020mpc, spahn2021coupled}. However, most MPC methods rely on convexification of the constraints and cost functions, which is inflexible for high-dimensional systems such as mobile manipulation. In addition, manipulation tasks often involve discontinuous contact and complex cost terms which are hard to differentiate analytically.

Sampling-based MPCs, such as MPPI \cite{williams2017information} and STORM \cite{bhardwaj2022storm}, offer promising alternatives. These algorithms make no restrictions on the convexity, non-linearity, discontinuity of the dynamics, and costs. The key idea of the algorithm is to sample control sequences from a given distribution and forward simulate them in parallel (e.g. on a GPU) using the system’s dynamics to generate trajectories. Each simulated trajectory is then evaluated against a cost function. The cost of each trajectory is then converted to update the distribution of control sequences. \textcolor{orange}{However, these works do not consider a sequence of plan switching as in TAMP plans. In \cite{abraham2020model}, the authors propose ensemble MPPI, a variation that handles complex tasks and adapts to parameter uncertainty, but the task modeling remains unclear and no open-source implementation is available.}

Interestingly, \cite{howell2022predictive} presents an open-source application based on MuJoCo physics for real-time predictive control. Among the challenges and future work, the authors suggested the use of learned policies when rolling out samples, and the use of a high-level agent to set the cost function of the predictive controller for long-horizon cognitive tasks. We follow this line of thought and propose a method to perform constraints composition for long-horizon tasks in a reactive fashion.  

% \paragraph{Controller fusion}

% to date, the field of controller fusion is largely unexplored, but past literature contains some early works using fuzzy logic \cite{fuzzyfusion, freire2002control, freire2004new, freire2001mobile, aycard1997new}. For instance, \cite{freire2002control} proposed to fuse different controllers' output for mobile robots. Hand-crafted fuzzy logic rules are used to associate a covariance to the each of the controllers depending on the situation a robot can encounter. The smaller this covariance the greater the influence of a controller. Authors in \cite{aycard1997new} also proposed to fuse behaviors through fuzzy logic, but again requiring several ad-hoc rules. 

% More recently, the authors in \cite{rana2020multiplicative} presented a Multiplicative Controllers Fusion approach. This method fuses a classical artificial potential field with a stochastic RL policy using their uncertainty to weigh their contribution to the control input. Follow-up work \cite{rana2021bayesian}, which also contains an extensive review of the state-of-the-art relvant for controller fusion, improved safety and performance in navigation and reaching behaviors compared to \cite{rana2020multiplicative}. However, stagnation of the control input can happen when the controller and policy are confident in different strategies. The same applies to \cite{baek2022hybrid}, where a hybrid learning and model-based controller is proposed by summing the torque output of a stochastic policy and a conventional LQR. 
% Alternatively, \cite{sharma2020learning} proposes using reinforcement learning to hierarchically compose object-centric controllers for manipulation tasks via nullspace projections. However, hierarchical projections can have discontinuities due to switching controllers, and adding new controllers would require re-training. 
% % Additionally, both \cite{rana2020multiplicative, rana2021bayesian} need a measure of the uncertainty of the controllers, which has to be artificially built for a deterministic controller.

% %\textcolor{blue}{Add works on RMPs}

% Finally, \textcolor{blue}{[ref elia]} showed how to include prior controllers as sample distributions for a
% model predictive path integral controller. This allowed to fuse an energy based controller with an LQR for a double pendulum swing-up, considering the controllers as rollouts in MPPI. This method has the potential of fusing an arbitrary number of controllers in a stochastic optimal control manner, but it lacks a way of handling long-horizon tasks.  

% In this work, we explore the potential of MPPI for controller fusion removing the need to compute the controller's and policy's uncertainties, and the risk of stagnation of the control input. Additionally, by using active inference for online decision making \cite{pezzato2022aipbt} to plan cost functions and select appropriate prior controllers, we achieve reactive TAMP where the MPPI can be applied throughout the whole task. 

% MPPI is a powerful sampling-based motion planner with a number of advantages but it cannot be applied for long-term tasks because of the limited horizon and the fact that the cost function would become complex and subject to local minima. 


% The solution of a TAMP problem is a finite sequence of high-level actions $\pi = [a_1,\ddots,a_k]$, and a set of continuous and discrete parameters that satisfy each action's constraints \cite{garrett2021integrated} and determine how an action is executed. The sequence of action templates is called \textit{plan skeleton}. Given a skeleton, the problem is then to select appropriate values so that the constraints of the
% actions in the skeleton are satisfied.

% In the concluding notes of \cite{garrett2021integrated}, future development of TAMP should focus on investigating novel strategies of combining optimization and sampling, as well as more realistic scenarios which include dynamics, and consider both state and action uncertainties. Finally, TAMP should focus on the inclusion of learning-based methods in order to require less human-provided domain knowledge. 

% It looks like TAMP is unable of making use of already available policies, since both task and motions are defined at planning time. One option would be to use a plan skeleton and blindingly execute the policy, this would be task planning and execution, the other would be to plan a trajectory, neglecting the available learned policy. So in TAMP we cannot make use of the vast amount of work for single skills learning, or use proven controllers developed over the years, instead we only stick to one optimization or sampling method for the motion planning part. 

